KGAT: Knowledge Graph Attention Network for Recommendation

To provide more accurate, diverse, and explainable recommendation, it is compulsory to go beyond modeling user-item interactions and take side information into account. Traditional methods like factorization machine (FM) cast it as a supervised learning problem, which assumes each interaction as an independent instance with side information encoded. Due to the overlook of the relations among instances or items (e.g., the director of a movie is also an actor of another movie), these methods are insufficient to distill the collaborative signal from the collective behaviors of users. In this work, we investigate the utility of knowledge graph (KG), which breaks down the independent interaction assumption by linking items with their attributes. We argue that in such a hybrid structure of KG and user-item graph, high-order relations --- which connect two items with one or multiple linked attributes --- are an essential factor for successful recommendation. We propose a new method named Knowledge Graph Attention Network (KGAT) which explicitly models the high-order connectivities in KG in an end-to-end fashion. It recursively propagates the embeddings from a node's neighbors (which can be users, items, or attributes) to refine the node's embedding, and employs an attention mechanism to discriminate the importance of the neighbors. Our KGAT is conceptually advantageous to existing KG-based recommendation methods, which either exploit high-order relations by extracting paths or implicitly modeling them with regularization. Empirical results on three public benchmarks show that KGAT significantly outperforms state-of-the-art methods like Neural FM and RippleNet. Further studies verify the efficacy of embedding propagation for high-order relation modeling and the interpretability benefits brought by the attention mechanism.

==> 1_introduction.tex <==
\section{Introduction}
Incorporating knowledge graphs (KGs) into recommender systems attracts increasing attention in both industry and academia~\cite{CKE,KGreasoning19,RippleNet,KGMemory18,KGRnn18}.
KG typically consists of real-world entities and the relations that hold between them.
% As such, the background knowledge of items is organized in the form of entity-relation-entity triplets, like (\emph{Hugh Jackman, IsCastOf, Logan}).
The structural knowledge is increasingly being used to work with user-item interactions in order to improve the accuracy and explainability of recommendation.

\begin{figure}[t]
    \centering
	\includegraphics[width=0.46\textwidth]{chart/intro.pdf}
% 	\vspace{-10pt}
	\caption{An illustration of collaborative knowledge graph and high-order connectivity for $u_1$.}
% 	The node $u_1$ is the target user to provide recommendations for.
	\label{fig:intro}
	\vspace{-10pt}
\end{figure}


Exploring user behaviors and item knowledge in a unified view, we are able to exhibit the relationship between users and items via the related entities and relations.
As illustrated in Figure~\ref{fig:intro}, the user of interest for recommendation is $u_1$ and her preferences on movie $i_3$ can be inferred by multi-hop relation paths:
\begin{itemize}%[leftmargin=*]
    \item $p_1: u_1\xrightarrow{r_1} i_1\xrightarrow{-r_1} u_2\xrightarrow{r_1} i_3$;
    
    \item $p_2: u_1\xrightarrow{r_1} i_1\xrightarrow{r_3} e_2\xrightarrow{-r_3} i_3$.
\end{itemize}
The multi-hop relation paths contains rich semantics that carries different \textbf{collaborative signal}.
To be more specific, $p_1$ attributes $u_1$'s choice on $i_3$ to the preferences of her similar user $u_2$.
Herein, $u_1\xrightarrow{r_1} i_1\xrightarrow{-r_1} u_2$ indicates the behavior similarity between $u_1$ and $u_2$; the longer path suggests that $u_1$ is likely to adopt $i_3$, since her similar user $u_2$ has consumed $i_3$ before.
This is consistent with the collaborative filtering (CF) effect --- similar users would exhibit similar preferences on items~\cite{BPRMF,NCF}.
Distinct from $p_1$, $p_2$ reasons about $u_1$'s interest to $i_3$ by her fine-grained preference on $e_1$.
Herein, $u_1\xrightarrow{r_1} i_1\xrightarrow{r_2} e_1$ suggests that $u_1$ might prefer movies acted by the actor $e_2$; we hence can recommend $i_3$ which has the same cast to her.
Such paths essentially use the semantic relatedness among items to augment the modeling of user-item interactions~\cite{CKE,DKN,CFKG}.
% As such, we believe that it is of crucial importance to model both collaborative effects in order to understand user preferences when consuming items.
How to effectively integrate different types of collaborative signal, while exploiting the compositional relations inside, is of crucial importance to augment the modeling of user-item interactions.

While many prior efforts on leveraging KG have been done~\cite{CKE,DKN,KGreasoning19,KGMemory18,DBLP:conf/icpr/Do0V18,KGreasoning19,KGRnn18}, it is challenging for them to achieve this goal.
A line of research~\cite{CKE,DKN,KGMemory18} encodes KG as embeddings and incorporates them into recommendation framework.
Nevertheless, they fail to exhibit the collaborative signal --- more specifically knowledge signal is transferred into semantic embeddings and CF signal is implicitly captured when reconstructing user-item interactions.
Moreover, the disregard of semantic relations within paths also limits their understanding of user preferences.
While extracting meta-paths~\cite{yu2013collaborative,DBLP:conf/wsdm/YuRSGSKNH14,DBLP:conf/ijcai/GaoYWZLH18,MetaFMG,Meta-path-2018kdd} or paths~\cite{KGreasoning19,KGRnn18}, another line model the user-item interactions largely upon the knowledge signal, leaving the CF signal untouched.
Besides, extensive domain knowledge is required to define meta-paths and labor-intensive feature engineering is needed to extract qualified paths.
Moreover, the scale of paths can easily reach millions or even larger in real-world scenarios, making it prohibitive to efficiently transfer high-quality knowledge in real-time.


More recently, RippleNet~\cite{RippleNet} is proposed to 


touched the idea of propagation, only items involved in paths rooted at a user are exploited to enrich her representations, where KG is leveraged only to construct multi-hop item candidates.
% It essentially combines path-based and neighbor-based methods, estimating the recommendation score based on the similarity between the target item and multi-hop items.
We hence argue that these approaches do not fully explore the high-order connectivity in the embedding space.



\section{Introduction}
Knowledge graphs (KGs) attract increasing attention to enhancing recommendation~\cite{CKE,KGreasoning19,RippleNet,KGMemory18,KGRnn18}.
KG typically provides a unified view of background knowledge related to items --- nodes are real-world entities and edges are relations that hold between them.
Transferring KG into recommender systems has a great potential to assist the representation learning of users and items, further augmenting the modeling of user-item 
relations.


Prior work on transferring knowledge as embeddings has been done~\cite{CKE,KGMemory18,DKN}.
The basic idea is to harness an item's (or a user's) representation by integrating knowledge embeddings derived from KG that are related to the item (or the user's historical items).
Herein, the knowledge embeddings capture entity semantics and make items with similar semantics close in the embedding space.
Such transferred knowledge mainly aims to inject item relatedness into recommendation framework, thereby guiding the representation learning of users and items.
For example, CKE~\cite{CKE} and DKN~\cite{DKN} combine embeddings of item self with that derived from KG triplets, and then optimize them via collaborative filtering.




These methods, however, are not sufficient to yield optimal embeddings for transferring knowledge into item recommendation.
The key reason is that the knowledge embedding function lacks an explicit encoding of crucial \textbf{collaborative signal}, which is inherent in user behaviors.
To be more specific, existing methods build the knowledge embedding function upon KG triplets only, while forgoing the interlinks between users, items, and entities (\eg as Figure~\ref{fig:intro} shows, $u_1$'s choices on $i_2$ \emph{X-Men} can be attributed to the cast $e_2$ \emph{Hugh Jackman}).
As a result, the resultant embeddings are suboptimal to reflect user behaviors and understand preferences on consuming items.



In this work, we propose the \textbf{collaborative knowledge graph} (CKG) --- more specifically the integration of user-item interaction graph and KG --- based on the alignment of entities and items.
We exploit the \textbf{high-order relational connectivity} of CKG, a natural way that represents collaborative signal, to improve the knowledge embedding and transferring processes.

% \begin{figure}[t]
%     \centering
% 	\includegraphics[width=0.46\textwidth]{chart/intro.pdf}
% % 	\vspace{-10pt}
% 	\caption{An illustration of collaborative knowledge graph and high-order connectivity for $u_1$.}
% % 	The node $u_1$ is the target user to provide recommendations for.
% 	\label{fig:intro}
% 	\vspace{-10pt}
% \end{figure}




\vspace{5px}
\noindent\textbf{Running Example}:
Figure~\ref{fig:intro} shows the concept of high-order relational connectivity, where the user of interest is $u_1$.
As the right subfigure shows, the tree structure rooted as $u_1$ consists of high-order relational connectivities, each of which denotes a path that reaches $u_1$ from any node with length $l$.
These connectivities express different multi-step relations, implying various compositional semantics:
1)~\emph{collaborative filtering signal}, which suggests that similar users would exhibit similar preferences on items (\eg $u_1\xleftarrow{r_1} i_1\xleftarrow{-r_1} u_2\xleftarrow{r_1} i_3$ indicates that $u_1$ is likely to adopt $i_3$, since her similar user $u_2$ has consumed $i_1$ before);
and 2)~\emph{collaborative knowledge signal}, which reveals fine-grained user preferences (\eg $u_1\xleftarrow{r_1} i_1\xleftarrow{r_2} e_1\xleftarrow{-r_2} i_3$ suggests that $u_1$ would adopt $i_3$ since it shares the same property $e_1$ with $i_1$ she liked before).
Furthermore, they are of varying importance to characterize user preferences.
An example of $u_1$'s preference on $i_3$ might by driven by the cast $e_2$ more than the producer $e_1$. 
Hence it is crucial to adaptively synthesize compositional semantics within high-order connectivity in order to embed and transfer knowledge effectively.





Although prior efforts on transferring such signal as meta-paths~\cite{yu2013collaborative,DBLP:conf/wsdm/YuRSGSKNH14,DBLP:conf/ijcai/GaoYWZLH18,MetaFMG,Meta-path-2018kdd} and paths~\cite{KGreasoning19,KGRnn18} have been done, it is highly challenging to achieve this goal because most of them require either extensive domain knowledge to predefine meta-paths, or labor-intensive feature engineering (\eg random walks) to extract qualified paths.
Moreover, the scale of paths can easily reach millions or even larger in real-world scenarios, making it prohibitive to efficiently transfer high-quality knowledge.






\vspace{5pt}
\noindent\textbf{Present Work}:
Instead of extracting paths, we design a neural network, \emph{Knowledge-Graph Attention Network} (KGAT), to propagate knowledge embeddings recursively on the collaborative knowledge graph.
It essentially passes messages along high-order relational connectivity in the embedding space.
Specifically, we devise an \textbf{attentive embedding propagation} layer, which updates the representation of each node (it can be user, item, and entity) by aggregating messages from the connected neighbors.
Wherein, the attention mechanism is introduced to specify the contribution of each neighbor for propagating embeddings towards the node, where the relation between them is considered to augment the semantic information.
By stacking multiple such layers, we are able to enforce the knowledge embeddings to capture the collaborative signal in high-order relational connectivity, getting rid of heavy feature engineering to extract paths.
For example, stacking two layers injects the behavior similarity of $u_1\xleftarrow{r_1} i_2\xleftarrow{-r_1} u_2$ and fine-grained preference of $u_1\xleftarrow{r_1} i_1\xleftarrow{r_2} e_1$ into $u_1$'s representations;
conducting three layers further captures the collaborative filtering and knowledge signals.
When performing the propagation of knowledge embeddings, we are able to extract the attention flow (which is an aggregation of attention scores between two nodes) and determine the explanation priority of connectivities.
As a result, we inject the collaborative signal into the knowledge embeddings for understanding user preferences on items. 
We conduct extensive experiments on three public benchmarks to verify the rationality and effectiveness of our method.



The contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*]
\item To the best of our knowledge, this is the first work that adopts graph neural networks to capture higher-order connectivity for effective knowledge-aware recommendation.

\item We develop a new framework, which encodes collaborative signal in the knowledge embedding function by transferring knowledge in the embedding space.

\item We conduct extensive experiments on three public benchmarks for top-N recommendation, showing significant improvements over the state-of-the-art methods.
% Empirical results indicate that using multiple propagation layers is capable of capturing the CF effect reflected in the higher-order connectivity.

\end{itemize}

==> 3_method.tex <==
\section{Model Framework}
We now formally present our RecKGN.
There are three components: (1) embedding layer to parameterize each node, while preserving the structural information of KG;
(2) attentive embedding propagation layers, which adopt the message-passing (\aka information propagation) architecture to inject high-order connectivity modeling into the embeddings, and specify the attention flow;
and (3) predict layer that assembles multiple propagated representations and outputs the matching score of a user-item pair.


% \begin{figure}[t]
%     \centering
% 	\includegraphics[width=0.44\textwidth]{chart/framework.pdf}
% 	\vspace{-10pt}
% 	\caption{Model Framework of RecKGN.}
% 	\label{fig:intro}
% 	\vspace{-15pt}
% \end{figure}


\subsection{Embedding}
% We represent the ID of user $u$, item $i$, and other entity $o$ with the embeddings $\Mat{e}_{u}, \Mat{e}_{i}, \Mat{e}_{o}\in\space{R}^{d}$, where $d$ is the embedding size.
% As a result, we establish the following embedding table:
% \begin{gather}\label{equ:e-0}
% 	\Mat{E}=[\underbrace{\cdots,\Mat{e}_{u},\cdots}_{\text{users}}, \underbrace{\cdots,\Mat{e}_{i},\cdots}_{\text{items}}, \underbrace{\cdots,\Mat{e}_{o},\cdots}_{\text{knowledge entities}}],
% \end{gather}
% which can be viewed as the latent features of entities to characterize their intrinsic information.
Following prior efforts~\cite{CKE,DKN}, we conduct TransR~\cite{TransR}, a KGE method, to parameterize each node (can be users, items, and other entities) and relation within KG, encoding semantic relatedness in the embeddings.
To be specific, for each triplet $(h,r,t)$, we represent the ID of head entity $h$, tail entity $t$, and relation $r$ with embeddings $\Mat{e}_{h}\in\Space{R}^{d}$, $\Mat{e}_{t}\in\Space{R}^{d}$, and $\Mat{e}_{r}\in\Space{R}^{k}$, where $d$ and $k$ are the embedding sizes of entity space and relation space, respectively;
in addition, we assign each relation with a transformation matrix $\Mat{W}_{r}\in\Space{R}^{d\times k}$, which projects entities from entity space into relation space.
At the core of TransR is the translation principle~\cite{TransR}: $\Mat{W}_{r}\Mat{e}_{h}+\Mat{e}_{r}\approx \Mat{W}_{r}\Mat{e}_{t}$, which makes representations of head entity $h$ and tail entity $t$ close in the space of relation.
For a given triplet $(h,r,t)$, its plausibility score can be formulated as follows:
\begin{align}\label{transr}
    g_{\Theta}(h,r,t)=\norm{\Mat{W}_{r}\Mat{e}_{h}+\Mat{e}_{r} - \Mat{W}_{r}\Mat{e}_{t}}_{2}^{2},
\end{align}
where $g(\cdot)$ with $\Theta$ as parameters is the scoring function.

Hereafter, we use pairwise loss of triplet ranking~\cite{CKE} to optimize the embedding learning process, which considers the relative order between correct and broken triplets.
Specially, the plausibility score of a correct triplet is expected to be larger than that of broken ones.
The loss function is as follows:
\begin{align}\label{equ:kg-loss}
    \Lapl_{\text{KG}}=\sum_{(h,r,t,t')\in\Set{T}}-\ln\mu\Big(g_{\Theta}(h,r,t)-g_{\Theta}(h,r,t')\Big),
\end{align}
where $\Set{T}=\{(h,r,t,t')|(h,r,t)\in\Set{G},(h,r,t')\not\in\Set{G}\}$, $(h,r,t')$ is the broken triplet by replacing one entity with another entity;
$\mu(\cdot)$ is the sigmoid function.
As a result, the semantic relatedness is encoded into the embeddings of entities, capturing the direct semantic relatedness among them.


\subsection{Attentive Embedding Propagation}
Next we build upon the message-passing architecture of graph convolution~\cite{GCN} and graph attention mechanism~\cite{GAT}, in order to propagate collaborative signals along the graph structure and enrich the representations of entities.

\subsubsection{\textbf{First-order Propagation}}
In terms of a user node, the historical items exhibit her preference distribution~\cite{FISM,SVDFeatures}.
In terms of an item node, the user group that consumes it can be treated as the item's features, which provides the behavior similarity of two items;
moreover, its facts describe it at aspect or feature level.
Analogous to other entity nodes, for example, the songs and albums profile a singer.
We build upon this intuition to perform information propagation between the connected user, item, and entity nodes.

We propose an attentive embedding propagation layer, which consists of three phases: \emph{message passing}, \emph{message attention} and \emph{message aggregation}.

\vspace{5px}
\noindent\textbf{Message Passing}.
For a triplet $\tau=(h,r,t)$, we parameterize the message being propagated from tail entity $t$ to head entity $h$ as an embedding:
\begin{gather}
    \Mat{m}_{\tau}=f_{\Theta}(\Mat{e}_{h},\Mat{e}_{t},p_{\tau}),
\end{gather}
where $f_{\Theta}(\cdot)$ with $\Theta$ as parameters is the information propagation, which takes $\Mat{e}_{h}$ and $\Mat{e}_{t}$ as inputs; and $p_{\tau}$ measures the importance of $t$ to $h$.
% where $\Mat{m}_{\tau}$ is the message embedding (\ie the information being propagated), and $f_{\Theta}(\cdot)$ with $\Theta$ as parameters is the information propagation function, which takes as input depends on the embeddings $\Mat{e}_{h}$ and $\Mat{e}_{t}$, and $p_{\tau}$ controls the decay factor on each propagation on edge $(h,r,t)$.
Here we follow graph convolution network (GCN)~\cite{GCN} and implement such propagation function using a linear transformation:
% In this work, we implement $f_{\Theta}(\cdot)$ using a linear transformation:
\begin{gather}\label{equ:0-message}
\Mat{m}_{\tau}=p_{\tau}\Mat{W}\Mat{e}_{i},
\end{gather}
where $\Mat{W}\in\Space{R}^{d'\times d}$ is the trainable weight matrix to distill useful information for propagation, and $d'$ is the transformation size.
% From the viewpoint of message passing, $p_{\tau}$ function can be interpreted as a discount factor, indicating the importance of the messages being propagated~\cite{DBLP:conf/icml/GilmerSRVD17}.

\vspace{5px}
\noindent\textbf{Attention Flow}.
In conventional message-passing architectures~\cite{RexGCN,GCMC,DBLP:conf/icml/GilmerSRVD17}, $p_{\tau}$ is typically set as $1/\sqrt{|\Set{N}_{h}||\Set{N}_{t}|}$.
Wherein, $\Set{N}_{h}$ and $\Set{N}_{t}$ denote the first-hop neighbor of node $h$ and $t$, respectively.
Such a heuristic setting depends only on the structure of graph, thus failing to specify varying importance scores of neighbors to the ego node~\cite{DeepInf}.
For example, a user may have different preferences on her historical items~\cite{ACF}, say, \emph{Alice} likes \emph{I See Fire} more than \emph{Shape of You};
similarly, the knowledge entities connecting an items have different contributes to profile it, say, \emph{Ed Sheeran} might carry more information than the release date when describing \emph{Shape of You}.
We hence argue that the such $p_{\tau}$ is not sufficient to yield optimal message embeddings.

Inspired by graph attention network (GAT)~\cite{GAT}, we introduce relational attention mechanism, which identities importance of each triplet and suggests parts of messages to focus on.
More formally, an attention coefficient $p_{\tau}$ is firstly computed as:
\begin{align}\label{equ:attention}
    p_{\tau}=\Trans{(\Mat{W}_{r}\Mat{e}_{t})}\rho\Big((\Mat{W}_{r}\Mat{e}_{h}+\Mat{e}_{r})\Big),
\end{align}
where $\Mat{W}_{r}\Mat{e}_{h}$, $\Mat{W}_{r}\Mat{e}_{t}$, and $\Mat{e}_{r}$ refer to the representations of $h$, $t$, and $r$ in the relation space, respectively;
$\rho(\cdot)$ is a nonlinear activation function set as tanh~\cite{GAT,Attention} here.
Distinct from traditional self-attention mechanisms~\cite{Attention} where attention coefficients between all possible node pairs will be computed, we only consider $a_{\tau}$ for $\tau\in\Set{G}$.
Furthermore, different from GAT which only takes representations of nodes as input, we model the relation between nodes.
By doing so, we not only preserve the structural information, but also allow adjusting the strength of propagation \wrt each triplet.
Note that, we employ only inner product on these representations for simplicity, and leave the further exploration of the attention module as the future work.

Hereafter, we normalize the coefficients across all triplets connected with $h$ by adopting softmax function:
\begin{align}
    p_{\tau}=\frac{\exp(p_{\tau})}{\sum_{\tau'\in\Set{G}_{h}}\exp(p_{\tau'})},
\end{align}
where $\Set{G}_{h}$ denotes the set of triplets where the head entity is $h$.
As a result, the final attention score is capable of suggesting which neighboring nodes should get more attention to capture CF signals.
When performing propagation forward, our attention flow suggests parts of the data to focus on, which can be treated as explanations behind the recommendation.

\vspace{5px}
\noindent\textbf{Message Aggregation}.
Having established the attentive messages, we can update the node's representation by assembling all messages.
Formally, we express the message aggregator $a(\cdot)$ as:
\begin{align}
    \Mat{e}^{(1)}_{h}=a(\Mat{e}_{h},\{\Mat{m}_{\tau}| \tau \in\Set{N}_{h}\}),
\end{align}
where $\Mat{e}^{(1)}_{h}$ is the updated representation of node $h$.
We employ a nonlinear transformation on the sum of incoming messages:
\begin{gather}\label{equ:1-aggregator}
	\Mat{e}^{(1)}_{h}=\sigma(\Mat{W}\Mat{e}_{h} + \sum_{\tau\in\Set{N}_{h}}\Mat{m}_{\tau}),
\end{gather}
where $\sigma(\cdot)$ is an activation function set as LeakyReLU~\cite{Nonlinear} here.
In addition to the messages passed from neighbors, we take the self-connection of $h$ into consideration: $\Mat{W}\Mat{e}_{h}$, which retains the information of original features.
To summarize, the advantage of the embedding propagation layer lies in explicitly exploiting the first-order connectivity information to relate user, item, and knowledge entity representations.

\subsubsection{\textbf{Higher-order Propagation}}
We further stack $l$ propagation layers to explore higher-order connectivity information, gathering the messages from the $l$-hop neighbors.
More formally, after $l$ steps, the representation of a node is recursively formulated as:
\begin{gather}\label{equ:l-aggregator}
    \Mat{e}_{h}^{(l)}=\sigma(\Mat{W}^{(l)}\Mat{e}^{(l-1)}_{h}+\sum_{\tau\in\Set{G}_{h}}\Mat{m}^{(l)}_{\tau}),
\end{gather}
wherein the message being propagated is defined as follows,
\begin{gather}\label{equ:l-message}
    \Mat{m}^{(l)}_{\tau}=p_{\tau}\Mat{W}^{(l)}\Mat{e}^{(l-1)}_{t},
\end{gather}
where $\Mat{W}^{(l)}\in\Space{R}^{d_{l}\times d_{l-1}}$ is the trainable transformation matrix, and $d_{l}$ is the transformation size;
$\Mat{e}_{t}^{(l-1)}$ is the item representation generated from the previous message-passing steps, memorizing the messages from its $(l$-1)-hop neighbors.
It further contributes to the representation of node $h$ at layer $l$, functioning as the indirect relatedness between the source and target nodes.

As Figure~\ref{xx} shows, the collaborative signal, such as like $u_{1}\xleftarrow{r_1} i_{2}\xleftarrow{r_3} e_{1}\xleftarrow{r_4} i_{4}$ and $u_{1}\xleftarrow{r_1} i_{3}\xleftarrow{r_2} u_{3}\xleftarrow{r_1} i_{4}$, can be captured in the embedding propagation process.
Furthermore, the message from $i_{4}$ is explicitly encoded in $\Mat{e}^{(3)}_{u_{1}}$ (indicated by the red line).
Clearly, the higher-order embedding propagation seamlessly injects the collaborative signals into the representation learning process.


\subsection{Model Prediction}

After performing $L$ layers, we obtain multiple representations for user node $u$, namely $\{\Mat{e}^{(1)}_{u},\cdots,\Mat{e}^{(L)}_{u}\}$;
analogous to item node $i$, $\{\Mat{e}^{(1)}_{i},\cdots,\Mat{e}^{(L)}_{i}\}$, is obtained.
As the output of $l$-th layer is the message aggregation of the tree structure depth of $l$ rooted at $u$ (or $i$) as shown in Figure~\ref{fig:intro}, the outputs in different layers emphasize different connectivity information.
We hence adopt the layer-aggregation mechanism~\cite{JumpKG} to concatenate the representations at each step into a single vector, as follows:
\begin{align}\label{equ:final-rep}
    \Mat{e}^{*}_{u}&=\Mat{e}^{(0)}_{u}\Vert\cdots\Vert\Mat{e}^{(L)}_{u},\nonumber\\
    \Mat{e}^{*}_{i}&=\Mat{e}^{(0)}_{i}\Vert\cdots\Vert\Mat{e}^{(L)}_{i},
\end{align}
where $\Vert$ is the concatenation operation.
By doing so, we not only enrich the initial embeddings by performing the embedding propagation operations, but also allow controlling the strength of propagation by adjusting $L$.

Finally, we conduct inner product of user and item representations, so as to predict their matching score, as follows,
\begin{align}
    \hat{y}(u,i)=\Trans{\Mat{e}^{*}_{u}}\Mat{e}^{*}_{i}.
\end{align}
In this work, we emphasize the embedding function learning, thus only consider the linear feature interaction between these two representations, leaving the exploration of nonlinear patterns in the future work.

\subsection{Optimization}

To optimize the recommendation module, we also opt for the BPR loss~\cite{BPRMF}.
Specifically, it assumes that the observed interactions, which indicate more user preferences, should be assigned higher prediction values than unobserved ones:
\begin{align}\label{equ:cf-loss}
	\Lapl_{\text{CF}}=\sum_{(u,i,j)\in\Set{O}}-\ln\mu\Big(\hat{y}(u,i)-\hat{y}(u,j)\Big)
\end{align}
where $\Set{O}=\{(u,i,j)|(u,i)\in\Set{R}^{+}, (u,j)\in\Set{R}^{-}\}$ denotes the training set, $\Set{R}^{+}$ indicates the observed (positive) interactions between user $u$ and item $j$ while $\Set{R}^{-}$ is the sampled unobserved (negative) interaction set;
$\mu(\cdot)$ is the sigmoid function.

Finally, we have the objective function to jointly learn Equations~\eqref{equ:kg-loss} and~\eqref{equ:cf-loss}, as follows:
\begin{align}\label{equ:loss}
    \Lapl_{\text{KGAT}}=\Lapl_{\text{KG}}+\Lapl_{\text{CF}}+\lambda\norm{\Theta}^{2}_{2},
\end{align}
where $\Theta$ is the model parameter set;
$L_{2}$ regularization parameterized by $\lambda$ on $\Theta$ is conducted to prevent overfitting.


\subsubsection{\textbf{Training.}}
We optimize $\Lapl_{1}$ and $\Lapl_{2}$ alternatively, where mini-batch Adam~\cite{xxx} is adopted to optimize the embedding loss and the prediction loss.
Adam is a widely used optimizer, which are able to adaptively control the learning rate \wrt the absolute value of gradient.
In particular, for a batch of randomly sampled $(h,r,t,t')$, we update the embeddings for all nodes; hereafter, we sample a batch of $(u,i,j)$ randomly, retrieve their representations after $L$ steps of propagation, and then update model parameters by using the garidents of the prediction loss.

\subsubsection{\textbf{Message and Node Dropout.}}
Although deep learning models have strong representation ability, they usually suffer from the overfitting.
Dropout is an effective solution to prevent neural networks from overfitting.
Following the prior work~\cite{GC-MC}, we adopt two dropout techniques: \emph{message dropout} and \emph{node dropout}.
Message dropout randomly drops out the outgoing messages.
In particular, we propose to adopt dropout on the messages being propagated in Equation~\eqref{equ:l-message}, with a probability $p_{1}$.
As such, in the $l$-th propagation layer, only part of messages contributes to the new representations.
We also conduct node dropout to randomly block a particular node and discard all its outgoing messages.
Especially, for the $l$-th propagation layer, we randomly drop $p_{2}$ percent on the nodes of the Laplacian matrix, where $p_{2}$ is the dropout ratio.

While the message dropout endows the representations more robustness against the presence or absence of single connections between users and items, node dropout focuses on reducing the influences of particular users or items~\cite{GC-MC}.
We perform experiments to investigate the role of message dropout and node dropout, analyzing their effectiveness in Section~\ref{sec:dropout}.



==> 5_related.tex <==
\section{Related Work}
We briefly introduce knowledge-aware recommendation methods.

\subsection{Regularization-Based Methods}
Prior efforts~\cite{CKE,KGreasoning19,RippleNet,KGMemory18} leverage KG triplets as a regularizer to guide the learning of user and item representations, while direct user-item connections are used to optimize the objective function for recommendation. For example, CKE~\cite{CKE} and DKN~\cite{DKN} generate semantic embeddings from KG via knowledge graph embedding (KGE) techniques, and then incorporate them into recommenders --- matrix factorization (MF)~\cite{BPRMF} and neural MF (NeuMF)~\cite{NCF}, respectively. Despite their great success, they only take direct connections between entities into consideration, while forgoing compositional relations within multi-hop paths. Such major limitation make them a suboptimal solution to transfer knowledge.

\subsection{Path-Based Methods}
%XN: can put in related work
Another line of research introduces meta-paths~\cite{yu2013collaborative,DBLP:conf/wsdm/YuRSGSKNH14,DBLP:conf/ijcai/GaoYWZLH18,MetaFMG,MCRec} and paths~\cite{KGreasoning19,KGRnn18} to directly infer user preferences. For instance, FMG~\cite{MetaFMG} and MCRec~\cite{MCRec} encode paths as embeddings to represent the user-item connectivity \wrt meta-paths; RippleNet~\cite{RippleNet} recently construct ripple set (\ie high-order neighboring items derived from KG) for each user to enrich her representations. While explicitly modeling high-order connectivity, it is highly challenging in real-world recommendation scenarios because most of these methods require extensive domain knowledge to define meta-paths or labor-intensive feature engineering to obtain qualified paths. Moreover, the scale of paths can easily reach millions or even larger when a large number of KG entities are involved, making it prohibitive to efficiently transfer knowledge.

% \subsection{Graph Neural Networks}
% Recently emerged graph neural networks (GNNs)~\cite{GCN,GraphSAGE,GAT} perform embedding propagation (or message passing) along the graph structure.
% At its core is the neighborhood aggregation, whcih 



% Recently emerged GNNs~\cite{GCN,JumpKG} offers us a chance to perform embedding propagation (or message passing) along the graph structure.
% At its core is the neighborhood aggregation, which iteratively aggregates the representations of each node with that of its adjacent nodes as its new representations.
% Inspired by the idea, researchers attempt to leverage GNNs to model high-order connectivity in recommender systems~\cite{GC-MC,SpectralCF,RM-GCN}.
% For example, RM-GCN~\cite{RM-GCN} performs random walks to generate the neighbors for items, and employs the graph convolutional networks~\cite{GCN} to update the item representations.
% SpectralCF~\cite{SpectralCF} considers the connectivity information in the spectral graph.
% However, these methods either need the random walk or suffer from the complexity issue, failing to fully explore the higher-order connectivity.

